SeRpEnt: Selective Resampling for Expressive State Space Models

State Space Models (SSMs) have recently enjoyed a rise to prominence in the field of deep learning for sequence modeling, especially as an alternative to Transformers. Their success stems from avoiding two well-known drawbacks of attention-based models: quadratic complexity with respect to the sequence length and inability to model long-range dependencies. The SSM variant Mamba has demonstrated performance comparable to Transformers without any form of attention, thanks to the use of a selective mechanism for the state parameters. Selectivity, however, is only evaluated empirically and the reasons of its effectiveness remain unclear. In this work, we show how selectivity is related to the sequence processing. Our analysis shows that selective time intervals in Mamba act as linear approximators of information. Then, we propose our SeRpEnt architecture, a SSM that further exploits selectivity to compress sequences in an information-aware fashion. It employs a resampling mechanism that aggregates elements based on their information content. Our empirical results in the Long Range Arena benchmark and other language modeling tasks show benefits of the SeRpEnt's resampling mechanism.

==> section_background.tex <==
\section{Background}
\label{sec:background}

\subsection{State Space Models}

State space models, a class of sequence transformation models, are defined through a set of first-order differential equations \emph{e.g.}, on real-valued functions $x (t) \in \sR \mapsto y (t) \in \sR$. Specifically, there exists a state vector $\vh \left(  \cdot \right) \in \sR^{N}$ such that the following equations are satisfied:

\begin{minipage}{0.45\textwidth}
\begin{subequations}
\begin{align}
    \dot{\vh}(t) & = \mA(t) \vh(t) + \mB(t) x(t), \label{eq:general_ssm_ode} \\
    y(t) & = \mC(t) \vh(t), \label{eq:general_ssm_output}
\end{align}
\end{subequations}
\end{minipage}
\hfill
\begin{minipage}{0.45\textwidth}
\begin{subequations}
\begin{align}
    \vh_{l} & = \overline{\mA}_l \vh_{l - 1} + \overline{\mB}_l x_l \label{eq:discrete_ssm_ode}, \\
    y_l & = \mC_l \vh_l \label{eq:discrete_ssm_output}
\end{align}
\end{subequations}
\end{minipage}

for matrices $\mA(t) \in \sR^{N \times N}$, $\mB(t) \in \sR^{N \times 1}$ and $\mC(t) \in \sR^{1 \times N}$, which are the state space parameters.

Equations (\ref{eq:discrete_ssm_ode}-\ref{eq:discrete_ssm_output}) express the case of discrete SSMs, where the input $x_l$ and output $y_l$ are $L$-length real-valued sequences rather than functions. In such case, we assume that the sequence $x_l$ is sampled from a continuous function $x \left( \cdot \right)$, where $x_l = x \left( t_l \right)$. Then, the discretized parameters $\overline{\mA}_l$, $\overline{\mB}_l$ are obtained using the zero-order hold \citep{pohlmann2010principles} rule as
\begin{equation}
\label{eq:zoh_disc}
\overline{\mA}_l = \exp({\Delta_l \mA}) ,~\textrm{and}~
\overline{\mB}_l = \left( \Delta_l \mA \right)^{-1} \left( \exp({\Delta_l \mA}) - \mI \right) \Delta_l \mB,
\end{equation}
where $\Delta_l = t_l - t_{l - 1}$ are the time intervals between sampling points.

\paragraph{LTI SSMs as recurrent and convolutional neural networks.} A continuous model is called a linear time-invariant (LTI) SSM when the parameters $\mA, \mB$, and $\mC$ are independent of time $t$. If we also assume constant time intervals $\Delta_l$ for the discrete LTI SSM model \emph{i.e.} the sequence $x_l$ is uniformly sampled from $x$, the equations (\ref{eq:discrete_ssm_ode}-\ref{eq:discrete_ssm_output}) can be simplified to

\begin{minipage}{0.4\textwidth}
\begin{subequations}
\begin{align}
    \vh_l & = \overline{\mA} \vh_{l - 1} + \overline{\mB} x_l, \label{eq:discrete_ltissm_ode} \\
    y_l & = \mC \vh_l, \label{eq:discrete_ltissm_output}
\end{align}
\end{subequations}
\end{minipage}
\hfill
\begin{minipage}{0.5\textwidth}
\begin{subequations}
\begin{align}
    \overline{K} & = (\mC \overline{\mB}, \mC \overline{\mA}^{1} \overline{\mB}, \dots, \mC \overline{\mA}^{l} \overline{\mB} ), \label{eq:kernel_conv} \\
    y & = x \ast \overline{K}. \label{eq:discrete_ssm_conv}
\end{align}
\end{subequations}
\end{minipage}

The model in (\ref{eq:discrete_ltissm_ode}-\ref{eq:discrete_ltissm_output}) can be interpreted as a RNN \citep{Yu2019ARO} with parameters $\overline{\mA}, \overline{\mB}$ and $\mC$. The transformations can also be computed as a convolution (\ref{eq:discrete_ssm_conv}) with the $\overline{K}$ kernel (\ref{eq:kernel_conv}). 
%\SR{Add a figure.}

\paragraph{Initialization of parameters.} HiPPO~\citep{gu2020hippo, gu2022train} demonstrates that the initialization of the state space parameters significantly impacts model performance. Their work derives expressions for $\mA$ and $\mB$ that enable an interpretation of the state vectors $\vh \left( \cdot \right)$ as coefficients for an approximation of $x \left( \cdot \right)$ on a polynomial space. Subsequent works \citep{gu2022parameterization, NEURIPS2022_9156b0f6, gu2022parameterization, Yu2023RobustifyingSM} propose $\mA$ simplification to speed up the computation of the kernel $\overline{K}$ in (\ref{eq:kernel_conv}). Particularly, our model relies on the structured SSM (S4) \cite{gu2022efficiently} approach, where the matrix $\mA$ is decomposed into a normal matrix $\mA_{\left( N \right)}$ and low-rank $\mP \mQ^{T}$ components ($\mP, \mQ \in \sR^{N \times 1}$) with the initialization as

\begin{minipage}{0.3\textwidth}
\begin{equation}
    \mA = \mA_{\left( N \right)} + \mP \mQ^{T},
\end{equation}
\end{minipage}
\hfill
\begin{minipage}{0.7\textwidth}
\begin{equation}
\mA^{\mathrm{init}}_{ij} = -
\begin{cases}
    \sqrt{2i + 1} \sqrt{2j + 1} & \text{if} i > j, \\
    i + 1 & \text{if} i = j, \\
    0 & \text{if} i < j.
\end{cases}
\end{equation}
\end{minipage}

\paragraph{Selective SSMs.}

While the initial line of work have been focused on LTI SSMs, Mamba~\citep{gu2023mamba} proposes to use the time-dependent parameters $\mB_l, \mC_l$ and $\Delta_l$. Then, the parameters are functions of the input $x_l$ that can be expressed by
\begin{equation}
\label{eq:mamba_deltan}
    \mB_l = \theta_{\mB} \left( x_l \right),~ 
    \mC_l = \theta_{\mC} \left( x_l \right),~\textrm{and}~
    \Delta_l = \mathrm{softplus} \left( \Delta + \theta_{\Delta} \left( x_l \right) \right),
\end{equation}
where $\theta_{\mB}$, $\theta_{\mC}$, $\theta_{\Delta}$ are linear transformations, and $\Delta_l$ is a learnable parameter. While the matrix $\mA$ is still time-invariant, the resulting $\overline{\mA}_l$ is not fixed because the discretization of $\mA$ depends on the time interval $\Delta_l$. In addition, the matrix $\mA$ is defined to be diagonal for efficiency reasons.

It is assumed that the sequence $x_l$ is sampled from an underlying continuous function $x ( \cdot )$. Then, $\Delta_l$ can be interpreted as time intervals between points $t_l$ at which the sequence elements are sampled as
\begin{equation}
    x_l = x \left( t_l \right) = x \left( \sum\nolimits_{i = 0}^{l} \Delta_i \right). \label{eq:time_intervals_sampling}
\end{equation}

% Possibly the main contribution of Mamba is the selectivity of the time-intervals $\Delta_n$ (as we will observe in the next section, the selectivity of $B_n$ and $C_n$ can be reinterpreted as a GLU non-linearity). That has both theoretical and practical implications.

% First, the authors of Mamba observe that, under simplified circumstances, the time-interval $\Delta_n$ acts as a gate for the update of the state vector $h_n$, hence reducing the model to a gated RNN. That means we can read $\Delta_n$ as a measure of relevance of the newly observed token $x_n$ compared to the previous $x_{n - 1}$.

% Second, because the model is not time-invariant anymore, we can not leverage the convolutional perspective in \ref{eq:discrete_ssm_conv} for concurrency. Instead, the use of as selective scan algorithm (also known as prefix sum) is employed to make the recurrence parallalizable, an approach first adopted for SSMs in the work of S5.

% Finally, we observe that a varying $\Delta_n$ equates to assuming the sequence $x_n$ is sampled non-uniformly from the underlying function $\tilde{x} \left( \cdot \right)$. More specifically, we assume that there exist $t_n \in \mathbb{R}$ with $t_n - t_{n - 1} = \Delta_n$ and

% \begin{equation}
%     x_n = \tilde{x} \left( t_n \right) = \tilde{x} \left( \sum_{i = 0}^{n} \Delta_n \right). \label{eq:nonuniform_sampling}
% \end{equation}

% Equation \ref{eq:nonuniform_sampling} might seem counter-intuitive with \ref{eq:mamba_deltan}, since we first express $\Delta_n$ in terms of $x_n$ and then the opposite. However, we emphasize that \ref{eq:nonuniform_sampling} is a purely theoretical device. In practice, it is not possible to obtain $x_n$ from it, because $\tilde{x}$ in unacessible.

\subsection{Learned Selectivity as a Linear Approximation of Information}
\label{sec:learned_selectivity_approx}

\cite{gu2023mamba} introduce selectivity as a strategy to improve the expressivity of SSMs. We extend their work by elucidating how the time intervals $\Delta_l$ learnt by Mamba serve as linear approximators of information contained in sequence elements $x_l$. We define the information in this context as the change in the conditional probability density function $p(y | \{ x_l \} )$ of an outcome $y$ for an observed sequence $\{ x_l \} = [ x_1, \ldots, x_i, \ldots, x_l ]$ and $l \leq L$, which we quantify as a difference in likelihoods with $(x_i \in \{ x_l \})$ and without $(x_i \not\in \{ x_l \})$ the $i$-th element. The effect of the change in likelihoods can be observed by studying the distribution $p ( y | \{ x_l \}_{l \neq i} )$ obtained by removing $x_i$ from the observations.

% but they left open the problem of justifying the effectiveness of the mechanism~(\ref{eq:mamba_deltan}). Here, we show that for a given sequence element $x_n$, the time interval $\Delta_n$ learnt by Mamba acts a linear approximator of information contained in $x_n$. We start by explaining what we mean by information contained in $x_n$.


% Given the two distributions $\mathcal{P} ( Y \; | \; \{ x_j \}_{j \leq L} )$ and $\mathcal{P} ( Y \; | \; \{ x_j \}_{j \neq i} )$, the information in $x_i$ can be formalized as a measure of the difference between the two, \emph{e.g.} in terms of Kullback-Leibler (KL) divergence:
% \begin{equation}
%     I \left(x_i, \left\{ x_j \right\}_{j \leq L} \right) = D_{\mathrm{KL}} \left( \mathcal{P} \left( Y \; | \; \left\{ x_j \right\}_{j \leq L} \right) \| \mathcal{P} \left( Y \; | \; \left\{ x_j\right\}_{j \neq i} \right) \right).
% \end{equation}

In the context of SSMs, the target distribution is modeled as a parametric one $p^\ast ( y^\ast | \vh_L )$ where $\vh_L$, the last state vector, is obtained from (\ref{eq:discrete_ssm_ode}). If $\vh_L^{i}$ denotes the last state vector obtained from the sequence $\left\{ x_l \right\}_{l \neq i}$, the distribution $p^\ast ( y^\ast | \vh_L^{i})$ is conditioned on the sequence without $x_i$. Thus, the information in $x_i$ can be quantified by the change between $p^\ast ( y^\ast | \vh_L )$ and $p^\ast ( y^\ast | \vh_L^{i})$.

In the context of information theory \citep{cover2012elements}, the difference between two distributions is usually measured as the Kullback-Leibler (KL) divergence. Because $p^{*}$ is parametric on $\bm{h}_L$ in a form that depends on the task and architecture at hand, we can not analytically express the KL divergence between $p^\ast ( y^\ast | \vh_L )$ and $p^\ast ( y^\ast | \vh_L^{i})$. However, on the assumption that all transformations involved are continuous (as they often are), the difference is related to the Euclidean distance between parameters $\| \vh_L - \vh_L^{i} \|$. That justifies the validity of the result in Proposition~\ref{prop:linear_inf_approx}.

% While $p^\ast$ is a function of $\vh_L$ in a way that it depends on the task and architecture at hand, we derive in Appendix~\ref{sec:app_selectivity} that the difference is related to the distance $\| \vh_L - \vh_L^{i} \|$ in Proposition~\ref{prop:linear_inf_approx} with the assumption that all involved transformations are continuous.

\begin{proposition} \label{prop:linear_inf_approx}
    For the discrete SSM defined by equations (\ref{eq:discrete_ssm_ode}-\ref{eq:discrete_ssm_output}) and (\ref{eq:zoh_disc}), when the matrix $\mA$ is diagonal, the distance $\| \vh_L - \vh_L^{i} \|$ is asymptotically linear with respect to $\Delta_i$ as $\Delta_i \to 0$ i.e.
    \begin{equation}
        \| \vh_L - \vh_L^{i} \| \sim c \Delta_i, \quad c=\mathrm{const}~\textrm{and}~\Delta_i \to 0.
    \end{equation}
\end{proposition}
\begin{proof}
    The proof is provided in Appendix \ref{app:app_selectivity}.
\end{proof}

%Then, we then have the following result, formalizing our claim that the time intervals $\{ \Delta_l \}_{l \leq L}$ in Mamba act as linear approximators of information.

We remark that the result does not depend on how $\Delta_i$ is obtained. Hence, we can tweak the function that computes the time intervals based on the behavior we are trying to model. In the next section,  we present our SeRpEnt and explain the benefits of computing $\Delta_i$ differently from Equation (\ref{eq:mamba_deltan}).

% \SR{Having to talk about Kullback-Leibler divergence and then resorting to distance is a bit inelegant, maybe we can do better by relating the KL divergence to the distance under suitably chosen decoding layers that do not break the asymptotic linearity? WIP. Also, it would help if we could add "We empirically support the result with some studies in the experiments section". WIP.}

==> section_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusions}

Inspired by our analysis of the selectivity mechanism, we introduced SeRpEnt, a method for compressing and decompressing sequences in SSMs. We showed how the time intervals learned by Mamba are linear approximators of information. This result justified the behavior of the proposed SeRpEnt that extends Mamba by compressing sequences in an information-aware fashion. We also showed SeRpEnt advantages empirically using the long-range arena benchmark and in other language modeling tasks. The proposed approach can benefit both current and future models when used as an architectural component that is orthogonal to the recent developments in other SSM variants.



\section{Acknowledgments}

The authors acknowledge financial support from the Panasonic Corporation and wish to thank the scientists at Panasonic for insightful discussions and recommendations.

\section{Data Availability Statement}

The data used to obtain the results of this paper can be obtained from the Long Range Arena repository \cite{tay2020long} and the Wikitext dataset \cite{merity2016pointer} accessible through the Hugging Face Hub.

==> section_experiments.tex <==
\section{Experiments}
\label{sex:experiments}

We empirically measure the performance of SeRpEnt on tasks of sequence classification and language modeling. In the first case, we evaluate SeRpEnt against a subset of the Long Range Arena (LRA) \citep{tay2020long} baselines, following previous works \citep{gu2022efficiently, gu2022parameterization, smith2023simplified}. In the second case, SeRpEnt is evaluated in language modeling using the experiment setup from \citet{fu2023hungry}.

All the details regarding experiments are reported in Appendix \ref{app:experimental_details}. We note here that we tested SeRpEnt against models with a comparable number of parameters. As explained in Section \ref{sec:serpent_architecture}, SeRpEnt is implemented independently from the SSM layer, which we apply depending on the task to: S4 \citep{gu2022efficiently} for LRA and Mamba \citep{gu2023mamba} for language modeling.

In our experiments, we observed that SeRpEnt improves the performance of the baseline it is applied on every task except for image ones in LRA. We believe the subset of image tasks in LRA (\textsc{Image}, \textsc{Pathfinder}, and \textsc{Pathfinder-X}) has a very different structural bias than the ones that sequence modeling problems manifest, and our experiments suggest SeRpEnt is incapable of capturing it. Exploring and justifying the shift in accuracy is cause for future research.

\subsection{Long Range Arena}

LRA is the benchmark composed of six sequence classification tasks which share one common property: modeling dependencies among distant sequence elements. Table \ref{tab:lra_table} shows results for SeRpEnt and other models the LRA tasks that involve sequence modeling, excluding those whose input are images. The reported score is accuracy. We are interested in comparing against an SSM architecture to its SeRpEnt variant. For reasons of completeness, we also report state-of-the-art results for models with quadratic complexity in the first three lines i.e. Mega \citep{ma2022mega}, ChordMixer \citep{khalitov2023chordmixer} and SeqBoat \citep{ren2023sparse}.

\setlength{\tabcolsep}{6pt}

\begin{table}[t]
    \centering
    \scalebox{0.88}{
        \begin{tabular}{m{3cm} m{1.4cm} m{1.4cm} m{1.7cm} | m{1.4cm}}
            \toprule
            {\centering \scalebox{1.2}{M}\small ODEL} & 
            {\centering \scalebox{1.2}{L}\small IST\scalebox{1.2}{O}\small PS} & 
            {\centering \scalebox{1.2}{T}\small EXT} & 
            {\centering \scalebox{1.2}{R}\small ETRIEVAL} & 
            {\centering \scalebox{1.2}{A}\small VG} \\ \midrule
            Mega & 63.14 & 90.43 & 91.25 & 81.01 \\ 
            ChordMixer & 59.89 & 88.87 & 90.38 & 79.71 \\ 
            SeqBoat & 61.70 & 89.60 & 91.28 & 80.86 \\ \midrule
            S4  & \textbf{59.60} & 86.82& 90.90 & 79.11  \\
            SeRpEnt+S4 & \textbf{59.60} & \textbf{88.60} & \textbf{91.18} & \textbf{79.79} \\
            \midrule
            S5  & 59.70 & 86.63 & \textbf{90.49} & 79.04  \\
            SeRpEnt+S5 & \textbf{60.35} & \textbf{89.62} &  89.04 & \textbf{79.67} \\
            \midrule
            Liquid-S4& \textbf{60.65} & 88.37 & 88.17 & 79.06 \\
            SeRpEnt+Liquid-S4 & 60.35 & \textbf{88.39} & \textbf{88.81} & \textbf{79.18} \\
            \bottomrule
            % \toprule
            % {\centering \scalebox{1.2}{M}\small ODEL} & 
            % {\centering \scalebox{1.2}{L}\small IST\scalebox{1.2}{O}\small PS} & 
            % {\centering \scalebox{1.2}{T}\small EXT} & 
            % {\centering \scalebox{1.2}{R}\small ETRIEVAL} & 
            % {\centering \scalebox{1.2}{I}\small MAGE} & 
            % {\centering \scalebox{1.2}{P}\small ATHFINDER} & 
            % {\centering \scalebox{1.2}{P}\small ATH-\scalebox{1.2}{X}} & 
            % {\centering \scalebox{1.2}{A}\small VG} \\ \midrule
            % % Attention Based Models
            % Mega & \textbf{63.14} & \textbf{90.43} & 91.25 & \textbf{90.44} & 96.01 & 97.98 & \textbf{88.21} \\ 
            % ChordMixer & 59.89 & 88.87 & 90.38 & 89.95 & \textbf{96.67} & \textbf{98.63} & 87.40 \\ 
            % SeqBoat & 61.70 & 89.60 & 91.28 & 90.10 & 96.35 & 96.68 & 87.62 \\ \midrule
            % % State Space Models
            % Liquid-S4 & \emph{62.75} & 89.02 & 91.20 & \emph{89.50} & 94.8 & 96.66 & 87.32 \\ 
            % % H3& 57.50 & 88.20 & 91.0 & 85.7 & 93.00 & 91.80 & 84.8 \\
            % S5 & 62.15 & \emph{89.31} & \emph{\textbf{91.40}} & 88.00 & 95.33 & \emph{98.58} & 87.46 \\ \midrule
            % S4 & \underline{59.60} & 86.82 & 90.90 & \underline{88.65} & \underline{94.20} & 96.35 & 86.09 \\ 
            % \textbf{SeRpEnt+S4} & \underline{59.60} & \underline{88.60} & \underline{91.18} & 86.24 & 82.35 & \underline{98.22} & \underline{86.78} \\ 
            % \bottomrule
        \end{tabular}
    }
    \caption{\textbf{Long Range Arena} Accuracy on individual LRA tasks  (excluding image ones) and the average, \%. Bold values denote an improvement from the baseline to SeRpEnt. On average, SeRpEnt shows a performance improvement over the base SSM models.}
    \label{tab:lra_table}
\end{table}

\subsection{Language Modeling}

For language modeling, at the time of writing, Mamba \citep{gu2023mamba} is the SSM variant with the best empirical performance. With the given computational resources at our disposal, we compare SeRpEnt+Mamba with a version of Mamba smaller than the ones evaluated in the original work and trained on WikiText-103-v1 \citep{merity2016pointer}, rather than the Pile \citep{pile}.

We train S4, Mamba, and our SeRpEnt on WikiText-103-v1 and report their performance metrics in Table \ref{tab:lm_table}. We observe that SeRpEnt outperforms Mamba despite the comparable number of parameters. This supports the efficacy of the proposed architecture. All models are trained on 4 Tesla V100 32Gb GPUs for a time ranging from two to four days.

With the size of the models and datasets in Table \ref{tab:lm_table}, we do not compare to large language model (LLM) baselines \citep{Zhao2023ASO}. However, these results support our claim that SeRpEnt introduces a positive impact on the Mamba architecture. To verify this, we meticulously match their hyperparameters to only measure the added performance as described in Appendix \ref{app:experimental_details}.

\begin{table}[h]
    \centering
    \scalebox{0.88}{
        \begin{tabular}{m{3cm} m{2cm} | m{2cm} m{2cm} m{2cm} m{2cm} m{2cm}}
            \toprule
            {\centering \scalebox{1.2}{M}\small ODEL} & 
            {\centering \scalebox{1.2}{M}\small ODEL \scalebox{1.2}{S}\small IZE} &
            {\centering \scalebox{1.2}{T}\small OP-1 ACC.$\uparrow$} & 
            {\centering \scalebox{1.2}{T}\small OP-5 ACC.$\uparrow$} & 
            %{\centering \scalebox{1.2}{T}\small OP5 \scalebox{1.2}{A}\small CCURACY$\uparrow$} & 
            {\centering \scalebox{1.2}{L}\small OSS$\downarrow$} & 
            {\centering \scalebox{1.2}{P}\small ERPLEXITY$\downarrow$} \\ \midrule
            S4 &  35.2M & 35.5 &  56.2 &  3.72 & 557 \\ 
            Mamba & 44.3M & 37.1 & 58.3 & 3.54 & \textbf{46} \\
            SeRpEnt+Mamba& 47.4M & \textbf{38.3} & \textbf{58.7} & \textbf{3.51} & \textbf{46}\\
            \bottomrule
        \end{tabular}
    }
    \caption{\textbf{Language Modeling on WikiText-103v1} The scores are for the dataset's test split. We compute performance metrics based on the official implementation of S4 and Mamba baselines. The proposed SeRpEnt's resampling mechanism with sequence compression improves the performance metrics (1.2\% and 0.4\% top-1 and top-5 accuracy, respectively) when added to the base model.}
    \label{tab:lm_table}
\end{table}
% \subsection{Experiment Setup}
% \subsection{Quantitative Experiments}

% \subsection{Qualitative Experiments}

\label{sec:experiments}

==> section_introduction.tex <==
\section{Introduction}
\label{sec:intro}

Sequence models, and more specifically language models, have gained the spotlight in the deep learning research due to their role as the backbone of foundational models (FMs) \citep{Achiam2023GPT4TR, Touvron2023LLaMAOA, Touvron2023Llama2O}. Overwhelmingly, their architecture is based on the Transformer \citep{NIPS20173f5ee243} with its attention mechanism \citep{bahdanau2014neural}. This approach is justified by the impressive body of empirical results in numerous applications \citep{ISLAM2024122666}. The Transformer, however, does not come without its own drawbacks. The attention layer enables the dense processing of elements in a sequence at the cost of a computational burden that scales quadratically with the context length. Besides the computational limitations, Transformers and sparse attention models \citep{child2019generating} are inefficient at modeling long-range dependencies, both empirically \citep{liu2023lost} and in \textit{ad-hoc} benchmarks \citep{tay2020long}.

State Space Models (SSMs) \citep{10.1115/1.3662552} are a class of models thoroughly studied in many established scientific areas. Recently, the HiPPO \citep{gu2020hippo} has paved the way in deep learning for sequence modeling by showing how SSMs can be leveraged for long-range dependencies with a careful initialization of the state parameters. Then, a class of SSM variants has been built on top of HiPPO, starting from the structured SSM (S4) \citep{gu2022efficiently} to, eventually, Mamba \citep{gu2023mamba}. The latter is the first SSM to match Transformers' performance without resorting to any form of attention. The main Mamba novelty is the selectivity, where state space parameters are themselves outputs of time-dependent neural networks \citep{45823hypernetorks}. While the idea is supported by compelling experiments, however, the source of its added expressivity is left unexplored with a room for further analytical and architectural exploration.

% SSMs rely on three properties that make them preferable over attention-based architectures. First, they are structured to process long sequences more effectively. Second, they enjoy a computational complexity that scales linearly with the sequence length. Finally, they exhibit a twofold interpretation: either as recurrent networks (RNNs) or as convolutional ones (CNNs). This duality of perspectives makes them fast in both online settings where elements are observed and processed one at a time (during inference in particular), and in parallel settings where the whole sequence is available from the start (during training).

% The advantage of SSMs over Transformers for long-range dependencies tasks was apparent from the start. For language modeling, however, it is only with Mamba that the architectures started outperforming attention-based models. Mamba accomplishes this with a selective mechanism, \textit{i.e.} by developing a time-dependant SSM with parameters depending on the sequence inputs through neural networks.

% \FG{The current second to fourth paragraphs are taking a long route. Fine to motivate the field of research as written in the first paragraph. Then, the second paragraph should pose the actual problem we're targeting, telling the current way of addressing it, and concluding with a statement of why it is not ideal/not what one should do/or currently not clear enough, thus demanding our analysis. Then, from a third paragraph on we start our main matter, our proposed model/analysis. An ideal third paragraph starts with "We propose". The one below is also a valid third paragraph if we focus on the task of understanding.}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{image_resampling.png}
    \caption{(\textbf{Top Left}) A linear time-invariant SSM with uniform sampling assumes a sequence $\{ x_l \}$ is sampled from an underlying continuous function which incurs a loss of precision due to the constant time interval $\Delta$. (\textbf{Top Right}) The Mamba computes time-variable intervals $\Delta_l$ that are dependent on the sequence elements: the sequence is assumed to be non-uniformly sampled from the underlying function. (\textbf{Bottom}) Our SeRpEnt assumes time-dependent intervals $\Delta_l$ and, additionally, resamples the sequence through interpolation by aggregating together elements whose information is related.}
    \label{fig:resampling}
\end{figure}

%  Alternative with caption on the side
% \begin{figure}[ht]
%     \centering
%     \begin{tabular}{ccc}
%         \begin{minipage}[c][5cm][c]{0.4\textwidth}
%             \centering
%             \includesvg[width=\textwidth, height=4cm]{images/figures/ssm.svg}
%         \end{minipage} &
%         \begin{minipage}[c][5cm][c]{0.4\textwidth}
%             \centering
%             \includesvg[width=\textwidth, height=4cm]{images/figures/mamba.svg}
%         \end{minipage} &
%         \multirow{2}{*}{\begin{minipage}[c][10cm][c]{0.2\textwidth}
%             \captionof{figure}{Lorem ipsum dolor sit amet, consectetur adipiscing elit, sed do eiusmod tempor incididunt ut labore et dolore magna aliqua. Ut enim ad minim veniam, quis nostrud exercitation ullamco laboris nisi ut aliquip ex ea commodo consequat. Duis aute irure dolor in reprehenderit in voluptate velit esse cillum dolore eu fugiat nulla pariatur. Excepteur sint occaecat cupidatat non proident, sunt in culpa qui officia deserunt mollit anim id est laborum.}
%         \end{minipage}} \\
%         \multicolumn{2}{c}{
%             \begin{minipage}[c][5cm][c]{0.8\textwidth}
%                 \centering
%                 \includesvg[width=\textwidth, height=5cm]{images/figures/serpent-resampler.svg}
%             \end{minipage}
%         } \\
%     \end{tabular}
% \end{figure}



% \SR{I think the value of better understanding the selective mechanism of Mamba and the model we proposed are comparable. I would, ideally, like a paragraph that emphasizes both and ties them together in the smoothest way possible.}


Stemming from a renewed analysis of the selectivity mechanism in Mamba, we propose \textbf{SeRpEnt}, a \textit{selective resampling procedure for sequence compression}. We show that selectivity learns to discriminate sequence elements based on amount of information in them. Using this analysis, SeRpEnt compresses sequences in an information-aware fashion: an overall reduction of the sequence length improves the global processing, while local elements are aggregated based on their information content. Figure \ref{fig:resampling} visualizes the main SeRpEnt novelty when compared to previous works.

% \FG{If we focus on understanding, then this paragraph starts well. If we propose SeRpEnt, then it's better to expose this in the first sentence of the paragraph, eg start with "Stemming from a renewed analysis of.. we propose SeRpEnt.."}

% In this work, we want to show how this fine-grained control can be exploited even further, developing sequence transformations that are capable of compressing or stretching the input at hand. \textbf{SeRpEnt}, the architecture resulting from this idea, brings advantages over previous SSMs. It allows for the model to restructure sequences based on their tokens' relevance, pruning when information is redundant and upsampling when inference is warranted. It also enables control over how the sequence length is processed, unlocking a potential for efficient compression that speeds up the training process. All of this is developed in a framework that fits neatly with the one of SSMs, showing how these are the natural backbone architecture for such a procedure.

% In other words, the source of Mamba's strong expressivity can be pinpointed to its fine-grained control over the sequence inputs, in contrast to previous SSMs that only allowed for global parameters shared across all sequence elements.

Our main contributions are summarized as follows:
\begin{itemize}
    \itemsep0em
    \item We show that selectivity is rooted in information processing capabilities, in particular the selective time intervals learned by Mamba act as linear approximators of information.
    \item We develop a selective resampling strategy for SSMs and propose our \textbf{SeRpEnt}, a model that compresses sequences in an information-aware fashion and, hence, enables more efficient global processing by aggregating together elements based on their information content.
    % \item We frame the selective resampling into a theoretical framework that fits into the extensive body of state spaces, providing a mathematical overview of the strategy's capabilities.
    \item We showcase SeRpEnt's performance in the Long Range Arena and other language modeling tasks to advance the development of SSMs as an alternative to Transformers.

\end{itemize}


==> section_method.tex <==
\section{Proposed Method}
\label{sec:method}

In this section, we describe SeRpEnt that compresses sequences before the application to a SSM. To do so, we leverage the two perspectives we develop for the time intervals $\Delta_l$: either as intervals between sampling points of the sequence (\ref{eq:time_intervals_sampling}) or as linear approximators of information in Section~\ref{sec:learned_selectivity_approx}.

% By decreasing the sequence length, SeRpEnt allows SSMs to better process global information. At the same time, it does so by leveraging the time intervals $\Delta_n$, ensuring a compression of the sequence that is information-aware.

% Selectivity unlocked a whole new degree of expressivity for SSMs, as Mamba proved itself to be the first competing model in language modeling without relying on attention. The mechanism, however, is explored only in a rudimentary way in the original paper. With SeRpEnt, we exploit selectivity to process compositional information, \emph{i.e.} information arising from consecutive elements in a sequence that compose into a shared block of meaning (for example, in the sentence "I went to the movies", the words "went to" compose to provide the shared meaning of "approaching a place").

% SeRpEnt works by leveraging the time intervals $\Delta_n$ computed selectively to resample the sequence $x_n$ into a compressed form $\overline{x}_n$, in which elements close enough together are aggregated into a shared state. The algorithm is summarized in Algorithm~\ref{alg:serpent}; in the following, we cover the details of the procedure.

% \begin{minipage}{0.5\textwidth}
% \begin{algorithm}[H]
% \caption{SeRpEnt} \label{alg:serpent}
% \hspace*{\algorithmicindent} \textbf{Input} $\text{sequence } x$ : $(B, L, H)$ \\
% \hspace*{\algorithmicindent} \textbf{Output} $y$ : $(B, L, H)$
% \begin{algorithmic}
%     \State $\Delta \gets \text{Parameter}$
%     \State $\Delta_n \gets \sigma \left( \theta_{\Delta} \left( x_n \right) \right) \Delta \left( 1 - \kappa \right) + \kappa \Delta$
%     \State $t_n \gets \sum_{i = 0}^{n} \Delta_n \text{ and } \overline{t}_n \gets n \Delta$
%     \State $\mathcal{N}_K \left( \overline{t}_n \right) \gets K \text{ closest neighbors in } \left\{ t_i \right\}_{i \leq L}$
%     \State $z_n \gets  \left[ \left( x_i, \varepsilon \left( \overline{t}_n - t_i \right) \right) \right] \text{ for } t_i \in \mathcal{N}_K \left( \overline{t}_n \right) $
%     \State $\overline{x}_n \gets \theta_{\Gamma} \left( z_n \right)$
%     \State $\overline{y} \gets \text{SSM} \left( \overline{x} \right)$
%     \State $y_n \gets \overline{y}_k \text{ with } k = \text{argmin}_{i} \left( t_n - \overline{t}_i \right)$
%     \State \textbf{return } $y + x$
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% \hfill
% \begin{minipage}{0.5\textwidth}
% \begin{algorithm}[H]
% \caption{SeRpEnt in Parallel} \label{alg:serpentpar}
% \hspace*{\algorithmicindent} \textbf{Input} $\text{sequence } x$ : $(B, L, H)$ \\
% \hspace*{\algorithmicindent} \textbf{Output} $y$ : $(B, L, H)$
% \begin{algorithmic}
%     \State $Y \gets \left[ \right] $
%     \State $Y$.append$\left(\text{SSM} \left( x \right) \right)$
%     \For{$i \gets 1, $ Number of SeRpEnt}
%     \State $Y$.append$\left( \text{SeRpEnt} \left( x\right) \right)$
%     \EndFor
%     \State $y \gets \text{Concatenate } Y$
%     \State $y \gets y + x$
%     \State \textbf{return } $y$
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}

\subsection{Sequence Compression}

Given a sequence $\left\{ x_l \right\}_{l \leq L}$, the length $L$ has a direct impact on the modeling capabilities of a SSM. A general input sequence is an element of $\ell^0 = \{ \{ x_l \}_{l \in \sN} \; | \; \exists L, \, \forall l > L, \, x_l = 0 \}$, the space of eventually-zero sequences. Because $\ell^0$ is infinite-dimensional, the outcome conditional distribution $p ( y | \{ x_l \}_{l \leq L} )$ is parameterized on an infinite-dimensional space. On the contrary, the predicted distribution $p^\ast ( y^\ast | \vh_L )$ of an SSM is parameterized on $\vh_L\in \sR^{N}$, a finite-dimensional representation of the whole sequence. Intuitively, the larger the length $L$, the less can be compressed into $\vh_L$, and, thus, the less expressive the SSM becomes.

The main motivation of this work is to compress an input sequence into a shorter one, while trying to incur a reduced loss of information. More formally, the problem can be described as follows.

\begin{problem}
    Given a sequence $\left\{ x_l \right\}_{l \leq L}$ and a length $\overline{L} < L$, find a sequence $\left\{ \overline{x}_l \right\}_{l \leq \overline{L}}$ such that the Kullback-Leibler (KL) divergence between $p ( y | \{ x_l \}_{l \leq L} )$ and $p ( y | \{\overline{x}_l \}_{l \leq \overline{L}} )$ is minimized.
\end{problem}

We propose a solution to the problem that combines heuristics with the result claimed in Proposition~\ref{prop:linear_inf_approx}. Then, we support the effectiveness of our approach empirically in Section \ref{sex:experiments}.

\subsection{Selective Resampling for Compression}
\label{sec:selective_resampling}

%\MM{Visto che alla fine SeRpEnt fa solo Pooling, non resampling, potremmo cambiare tutti i "Resampling" in "pooling" cosí da essere piú chiari. Se non erro questa cosa era uscita anche nelle review}

\begin{figure}
\includegraphics[width=0.95\linewidth]{image_Serpent.png}
\caption{(\textbf{Compression}) During the compression procedure through selective resampling a time interval $\Delta_l$ is computed for each element $x_l$ of the sequence. Then, the intervals are used to obtain the times at which elements sampled from the underlying function. Based on the $\Delta_l$ value and $\Delta$, elements are resampled and processed with a linear transformation together with their $K$ closest neighbors. Finally, the compressed sequence is the input to a SSM.}
\label{fig:serpent}
\end{figure}

As in Mamba, we start by computing a time interval value $\Delta_l$ for each $x_l$ in the sequence. From the discretization perspective, the time intervals are related to the times $t_l$ at which elements $x_l$ are sampled from the underlying continuous function $x\left( \cdot \right)$ in (\ref{eq:time_intervals_sampling}). In addition, Proposition~\ref{prop:linear_inf_approx} states that the $\Delta_l$ are related to the information contained in the elements $x_l$. This motivates our idea: to compose elements together based on their information content, \emph{i.e.} the value of $\Delta_l$.

In practice, we resample the sequence $\left\{ x_l \right\}_{l \leq L}$ into a compressed one $\left\{ \overline{x}_l \right\}_{l \leq \overline{L}}$ in which close elements are composed together. We achieve this by taking $\overline{x}_l$ to be uniformly sampled from the same underlying function:
\begin{equation}
    \overline{x}_l = x \left( \overline{t}_l \right) = x \left( l {\Delta} \right),
\end{equation}
where the $\overline{t}_l$ are the resampled times with a constant time interval ${\Delta} = \overline{t}_l - \overline{t}_{l - 1}$. Since we can not access the underlying function $x \left( \cdot \right)$, we infer $\overline{x}_l$ through interpolation.

For both $x_l$ and $\overline{x}_l$, we know the times at which they are sampled from $x \left( \cdot \right)$: $t_l = \sum\nolimits_{i = 0}^{l} \Delta_i$ and $\overline{t}_l = l \Delta$, respectively. This enables the adoption of a nearest neighbors procedure \citep{hastie2009elements} for interpolation. Given a window size $K$, for each $\overline{t}_l$, $\mathcal{N}_{K} \left( \overline{t}_l \right)$ is the set of the its $K$ closest neighbors among the input times $\left\{ t_l\right\}_{l \leq L}$. The interpolation procedure infers $\overline{x}_l$ as a function $\Gamma$ of its nearest neighbors.

% \begin{equation}
% \label{eq:gamma_interpolation}
%     \overline{x}_l = \Gamma \left( \left\{ \left(x_k, t_k \right) \; | \; t_k \in \mathcal{N}_K \left( \overline{t}_l \right) \right\} \right).
% \end{equation}

Figure \ref{fig:serpent} illustrates the compression operation in our method. In particular, we select $\Gamma$ to be a linear transformation $\theta_{\Gamma}$ applied on the concatenation $\bigoplus$ of the inputs $x_k$ and their processed distances $\varepsilon \left( \overline{t}_l - t_k \right)$ from the resampled point can be expressed as
\begin{subequations}
\begin{align}
    \overline{x}_l & = \Gamma \left( \left\{ \left(x_k, t_k \right) \; | \; t_k \in \mathcal{N}_K \left( \overline{t}_l \right) \right\} \right) \label{eq:gamma_interpolation}, \\
    \overline{x}_l & = \theta_{\Gamma} \left( \bigoplus\nolimits_{t_k \in \mathcal{N}_K \left( \overline{t}_l \right)} \left[ x_k, \varepsilon \left( \overline{t}_l - t_k \right)\right] \right) ~\textrm{with }~ \varepsilon \left( d \right)_i = \exp(-\left( d - \mu_i \right)^2). \label{eq:linear_interpolation}
\end{align}
\end{subequations}

\paragraph{Gaussian basis expansion of time differences.}

We borrow a trick from the literature of graph neural networks \citep{NIPS2017_303ed4c6} to represent the time differences $d_{lk} = \overline{t}_l - t_k$. If the time difference is processed as a scalar, the random initialization of linear layers makes the information processed at different distances highly correlated. To avoid that, we expand the time difference $d_{lk}$ in a vector of Gaussian coefficients $\varepsilon ( d_{lk} )$ (\ref{eq:linear_interpolation}) where the means $\left\{ \mu_i \right\}_{i \leq G}$ are randomly initialized and learnable, while the dimension $G$ of the expansion is a hyperparameter of the model.

\paragraph{Resampling and compression rate.}

The most important component of the resampling procedure is the computation of the time intervals $\Delta_l$. The computation must ensure that the output sequence is a compression of the input, which is guaranteed if $\Delta_l \leq \Delta$. A hyperparameter $0 < \kappa < 1$ also controls the minimum compression rate, \emph{i.e.} $\overline{L} \geq \kappa L$, which can be ensured by posing $\Delta_l \geq \kappa \Delta$. We then employ the following expression for computing the time intervals
\begin{equation}
\label{eq:delta_serpent}
    \Delta_l = \sigma \left( \theta_{\Delta} \left( x_l \right) \right) \Delta \left( 1 - \kappa \right) + \kappa \Delta,
\end{equation}
where $\sigma$ is the sigmoid function, $\theta_{\Delta}$ is a linear transformation, and $\Delta$ is a learnable parameter. Because $0 < \sigma ( \theta_{\Delta} ( x_l ) ) < 1$, we have $\kappa \Delta \leq \Delta_l \leq \Delta$.

% \paragraph{Causal resampling.}

% For a given resampled time $\overline{t}_n$, the set $\mathcal{N}_K \left( \overline{t}_n \right)$ draws from both points before and after $\overline{t}_n$. This makes the resampling operation non-causal and suited for sequence classification, but not for tasks like language modeling. For causal tasks, we constrain the nearest neighbors $\mathcal{N}_K \left( \overline{t}_n \right)$ to be drawn exclusively from points before $\overline{t}_n$, so we avoid accessing information that would not be available at inference time.

\subsection{SeRpEnt Architecture}
\label{sec:serpent_architecture}

We have described the inner functioning of the selective resampling procedure for compression of a sequence $\{ x_l \}_{l \leq L}$ into $\{ \overline{x}_l \}_{l \leq \overline{L}}$. We now present how that fits into the overall architecture of SeRpEnt. We remind that the choice of $\kappa$ in equation (\ref{eq:delta_serpent}) tunes the compression rate of the resampling procedure. Then, our SeRpEnt block compresses a sequence at different compression rates $\kappa_b$ and applies a separate SSM to each of them. Finally, each output sequence is decompressed and all of them are concatenated together. We further explain these steps in details with the overall architecture being depicted in Figure \ref{fig:serpent_arch}.

\begin{figure}
\includegraphics[width=0.95\linewidth]{image_parallel.png}
\caption{(\textbf{Architecture}) Our SeRpEnt block works by compressing an input sequence $\{ x_l \}_{l \leq L}$ at different compression rates. It separately processes each of the compressed inputs using a SSM layer, decompresses the outputs, and concatenates them back into a single sequence with a skip connection.}
\label{fig:serpent_arch}
\end{figure}

\paragraph{Compression through selective resampling.} In each $b$-th SeRpEnt block, we perform this operation as covered in Section \ref{sec:selective_resampling}, in parallel for all blocks, with different compression rate $\kappa_b$. Hence, the input of this component is the sequence $\{x_l\}_{l \leq L}$ and its output is a series of compressed sequences $\{\overline{x}_l^b\}_{l \leq \overline{L}^{b}}$, one for every compression rate. This allows us to efficiently model short- and long-range dependencies by aggregating together elements based on their information content.

\paragraph{State space model.}
A SSM processes each compressed sequence $\{ \overline{x}_l^b \}_{l \leq \overline{L}^{b}}$ to obtain output sequence $\{ \overline{y}_l^{b} \}_{l \leq \overline{L}^{b}}$ with the the same length. We emphasize that SSM choice is independent from our resampling procedure. Therefore, our method can serve as an architectural extension for other SSM layer variants. We leverage this in the Section \ref{sec:experiments} experiments.

\paragraph{Reverse resampling.}
This step decompresses the sequences $\{ \overline{y}_l^{b} \}_{l \leq \overline{L}^{b}}$ to the original length $L$. Formally, for each individual $\{\overline{y}_l^{b} \}_{l \leq \overline{L}^{b}}$, the operation is equivalent to the compression one, but with the original and the resampled times being inverted. For each output time $t_l$, we find its nearest neighbors $\mathcal{N}_K (t_l)$ among $\{ \overline{t}_l \}_{l \leq \overline{L}}$ and express $y_l$ as a function $\Gamma^{*}$ of $\{ (\overline{y}_k, \overline{t}_k) \; | \; \overline{t}_k \in \mathcal{N}_K (t_l) \}$ from equation (\ref{eq:gamma_interpolation}). In practice, we find $\Gamma^{*}$ to work well by simply copying the closest $\overline{y}_k^b$ to $y_l$. The following equations recap all the operations in the SeRpEnt block:

\begin{minipage}{0.6\textwidth}
\begin{subequations}
\begin{align}
    \overline{x}^b_l & = \theta_{\Gamma} \left( \bigoplus\nolimits_{t_k \in \mathcal{N}_K \left( \overline{t}^i_l \right)} \left[ x_k, \varepsilon \left( \overline{t}^b_l - t_k \right)\right] \right), \\
    y^b_l & = \overline{y}^b_k \textrm{ with } k = \textrm{argmin}_{j} \left| t_l - \overline{t}_j^b \right|,
\end{align}
\end{subequations}
\end{minipage}
\hfill
\begin{minipage}{0.3\textwidth}
\begin{subequations}
\begin{align}
    \overline{y}^b & = \textrm{SSM} \left( \overline{x}^b \right), \\
    y_l & = \left( \bigoplus\nolimits_b y_l^b \right) + x_l.
\end{align}
\end{subequations}
\end{minipage}

Overall SeRpEnt network is a concatenation of individual blocks. We do not interleave blocks with linear layers due to the fact that features get linearly mixed during the resampling step in (\ref{eq:linear_interpolation}).

% \subsection{SSM and Reverse Resampling}

% Once we have obtained the resampled sequence $\overline{x}$ from $x$, we apply an SSM to it. We remark that the choice of the SSM is independent from the resampling procedure, allowing for an improvement to existing architectures that is orthogonal to the development of new SSM layers. In our research, we choose to work with either S4 or Mamba as the SSM block, depending on the task at hand.

% After the application of the SSM layer, we obtain an output $\overline{y}$ with the same length $\overline{L}$ as $\overline{x}$. In order to have an output with the same length $L$ as the original sequence $x$, we revert the resampling operation on $\overline{y}$. This allows us to apply skip-connections as well as to have an output per element at the end of the model, useful for language modeling tasks.

% For the reverse resampling, we mostly follow the same procedure as the forward one, this time working with inverted input and resampled times. One crucial difference for the reverse resampling is that we do not use any linear transformation for the interpolation of elements, instead we simply copy the closest $\overline{y}_k$ for each element $y_n$. This is in line with the interpretation of the resampled elements as states of composed information: if $\overline{y}_k$ aggregates the information for $y_{k_1}, \hdots, y_{k_j}$, than the state should be shared across such elements.

% \subsection{Parallel SeRpEnt}

% To summarize, the structure of a SeRpEnt block is the one in algorithm \ref{alg:serpent}. A complete deep architecture consists of several blocks one after each other. Because the resampling operation already processes interactions between features, we do not interleave blocks with linear layers, as those would introduce redundant hyperparameters. In addition to that, given that most SSM layers already incorporate non-linearities, we also avoid interleaving them.

% One advantage of SeRpEnt, which we have found effective in experiments, is that different SeRpEnt blocks can be applied in parallel with different compression ratios, rather than just sequentially. This allows to process compositional information at different levels of frequency. The procedure is explained in algorithm \ref{alg:serpentpar}.  

% {\color{red}
% \begin{theorem}
%     Given a function $f : \mathbb{R} \to \mathbb{R}$, under constraints, the maximum amount of information from a discrete sampling is achieved with uniform sampling $f \left( n \Delta \right)$ (under a suitable distribution defined on a regular enough function space...)
% \end{theorem}

% \begin{theorem}
%     A state space model $s : \mathcal{F} \to \mathcal{F}$ achieves the minimum discretization error when working on uniformly sampled sequences.
% \end{theorem}
% }

==> section_related.tex <==
\section{Related Work}
\label{sec:related}

% \LF{Each section has to follow a top-down approach. \\ We should start with the problem that SSMs solve, that is, long-range dependencies. Then, briefly explain why the first SSM was introduced and how it solved the problem. Following, explain what the following models improved and what they introduced (in 1 or 2 sentences).\\ Finally, conclude what is the actual problem of the SOTA model and briefly explain what is our solution and why this is novel compared to the SOTA. This last sentence should be a "repetition" of the novelty introduced in the Intro.}

Despite progress in the field of machine learning for sequence processing \citep{Lim2020TimeseriesFW}, capturing long-range dependencies has proven a difficult problem to tackle \citep{CHEN2023101819}.  Particularly, this is evident in scenarios characterized by large contextual windows in the domain of Natural Language Processing (NLP) \citep{manning1999foundations}, where the retrieval of specific information in large textual corpora presents a challenging task \citep{khandelwal2018sharp, kandpal2023large}. In this section, we review recent mainstream approaches for the problem of modeling long-range dependencies. We discuss their properties and rationale, as well as their shortcomings.

\subsection{Attention Mechanism in Transformers}
% - attention is good but has two main problems: quadratic computational time and long-range dependencies;  \\
% - the first problem was approached by reducing the computational limit below the "quadratic time" (flash attention, sparse attention ...); \\

The attention mechanism \cite{bahdanau2014neural, NIPS20173f5ee243} has become ubiquitous in sequence modeling, thanks to its capability of relating tokens in a sequence. That justifies approaches for long-sequence modeling built upon its cornerstone architecture: the Transformer. However, the Transformer presents a dual problem in the specific context of long-range dependencies: the computational complexity of inferring a token is quadratic in the length of the sequence, and its expressivity is negatively affected when applied to long sequences \citep{liu2023lost, li2024longcontext}. 

To overcome the first shortcoming, alternative forms of attention have been proposed \citep{wang2020linformer, kitaev2020reformer, child2019generating}, which rely on sparse representations and computations. More recently, \cite{dao2022flashattention} develop a fast implementation which exploits the GPU hardware to minimize data exchange. While sparse attention successfully deals with the computational side of the problem, their second drawback, \emph{i.e.} the expressivity for modeling long-range sequences, remains a major obstacle in many practical applications \citep{zhang2023cab}.

\subsection{State Space Models}
% - however, the second problem is not solved by these models, and here come the SSMs (S4, S5, mamba, ...) to solve both; \\
% - finally, identify a lack/problem of mamba and then say what novelty we propose compared to mamba.}

State space models are an established family of transformations in traditional statistics. The authors of HiPPO \citep{gu2020hippo} propose the use of SSMs as an alternative backbone for long sequence modeling by leveraging a theory for parameters initialization. Unlike transformers, this approach unlocks inference with linear complexity. \cite{gu2022efficiently} further suggests an efficient convolutional approximation for SSMs which enables concurrent computations at training time. The initial success of SSMs spurred a research in related areas \emph{e.g.} audio generation \citep{pmlr-v162-goel22a}, reinforcement learning \citep{lu2023structured}, and spatiotemporal modeling \citep{smith2023convolutional}.

\cite{fu2023hungry} are the first to explore the use of SSMs for language modeling. More recently, Mamba \citep{gu2023mamba} proposes the first SSM capable of matching Transformer's performance in the NLP tasks. Mamba does so by removing the linear time-invariant constraint in previous works and by using a time-dependent parametric selectivity mechanism. This leads to a fully recurrent model that generalizes prior gated recurrent units \citep{Cho2014LearningPR}. Authors argue that the main source of improvement comes from the model being able to selectively update its memory and decide which information to discard and which to retain. The arguments, however, are only explored empirically and the lack of an appropriate framework for understanding and exploiting the selectivity mechanism spurs future research, including this work.

Mamba spurred an extensive following of works that build upon it \citep{mamba2}, in some cases adapting it to other types of data \citep{liang2024pointmambasimplestatespace, xie2024quadmamba}. The authors of \citep{zhan2024exploringtokenpruningvision} propose to extend Mamba with a token pruning mechanism that resembles our compression strategy. In our case, however, we do not apply direct pruning, but process every token to obtain a shorter sequence to process.

% introduced a non-LTI SSM which used a hardware aware algorithm to efficiently compute recurrences inspired by \citet{dao2022flashattention}. \LF{Explain the main contribution of mamba, which should be the selection mechanism and provide the high-level intuition behind it. \\ At this point, we have presented the actual scenario, and we should emphasize the problem that no one has already solved and for which we are proposing the paper. Briefly explain the problem in one sentence and mention, in the following sentence, our novelty (as a high-level concept).}
% It has been argued that the selectivity mechanism of SSMs is key to the expressivity of the model, and this inspired us to further develop this concept.



% In order to 
% State Space Models have become an interesting \LF{"interesting" is generic, start with the problem} field of study since \citet{gu2023mamba} has showed their competitiveness against the transformer architecture \citep{NIPS2017_7181}. In particular, \ showed the struggle of transformers to keep up with long-range dependencies, and this started the research on equally expressive alternative architecture \LF{This sentence should be the first one, but briefly introduce the framework: "Capture long-range dependencies represents a foundational problem in machine learning, particularly evident in scenarios characterized by large contextual windows. Within the domain of Natural Language Processing (NLP), the retrieval of specific information within large textual corpora presents a challenging task [ADD REFs]. Analogously, in the context of forecasting, it is critical to discern patterns within long temporal sequences [ADD REFs]."}.
% \LF{Here add proof of this problems in the specific domain of long range dependencies, such as \citet{liu2023lost} and \citet{tay2020long}. Then introduce the first SSM.}



% Early studies on the HiPPO matrix started Linear Time-Invariant SSMs that could retain and compress memory of the input \citep{gu2020hippo}. 
% This work was further expanded by S4 \citep{gu2022efficiently} which implemented an efficient approximation of this process. 
% S4D \citep{gu2022parameterization} and S5 \citep{smith2023simplified} independently discovered that a diagonal approximation of the HiPPO matrix is still able to retain memory, and the latter also implemented an efficient parallel scan which used a MIMO approach rather than a SISO as its predecessors. \LF{The focus in the explanation of these models should be on their novelties more than their engineering for improved efficiency.}


